Cohmeleon: Learning-Based Orchestration of Accelerator Coherence in Heterogeneous SoCs

One of the most critical aspects of integrating loosely-coupled accelerators in heterogeneous SoC architectures is orchestrating their interactions with the memory hierarchy, especially in terms of navigating the various cache-coherence options: from accelerators accessing off-chip memory directly, bypassing the cache hierarchy, to accelerators having their own private cache. By running real-size applications on FPGA-based prototypes of many-accelerator multi-core SoCs, we show that the best cache-coherence mode for a given accelerator varies at runtime, depending on the accelerator's characteristics, the workload size, and the overall SoC status. Cohmeleon applies reinforcement learning to select the best coherence mode for each accelerator dynamically at runtime, as opposed to statically at design time. It makes these selections adaptively, by continuously observing the system and measuring its performance. Cohmeleon is accelerator-agnostic, architecture-independent, and it requires minimal hardware support. Cohmeleon is also transparent to application programmers and has a negligible software overhead. FPGA-based experiments show that our runtime approach offers, on average, a 38% speedup with a 66% reduction of off-chip memory accesses compared to state-of-the-art design-time approaches. Moreover, it can match runtime solutions that are manually tuned for the target architecture.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

SRCS = paper.tex
PDFS = ${SRCS:%.tex=%.pdf}

RM = rm -rf

# Dependencies
SECTIONS = $(wildcard sections/*.tex)
FIGURES = $(wildcard figures/*.eps) $(wildcard figures/*.pdf)
GRAPHS = $(wildcard graphs/*.eps) $(wildcard graphs/*.pdf)

all:  ${PDFS}

%.pdf:  %.tex paper.bib $(SECTIONS) $(FIGURES) $(GRAPHS) acmart.cls ACM-Reference-Format.bst
	pdflatex $<
	@if test -f $(@:.pdf=.aux) &&  test `grep citation $(@:.pdf=.aux) | wc -l` -ge 1; then bibtex $(@:.pdf=); fi
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.pdf auto


.PHONY: all %.pdf clean


==> sections/artifact.tex <==
\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

To build and evaluate \cohmeleon, we leveraged ESP, an open-source platform for
agile design and prototyping of heterogeneous SoCs. We integrated \cohmeleon in
ESP, and we released it in a fork of ESP on GitHub. \cohmeleon will be merged
into the main ESP repository on GitHub before MICRO 2021.

We collected the results presented in the paper by running real-size
applications on FPGA-based prototypes of many-accelerator multi-core SoCs
designed with ESP. The main steps required to evaluate \cohmeleon on FPGA
include: high-level synthesis (HLS) of accelerators, FPGA bitstream generation
for full SoCs, software build, deployment of the SoCs and software on an FPGA
board, and execution of the experiments on the FPGA by running application
software on top of the Linux operating system. This document contains the
instructions for reproducing the experiments presented in the paper.


\subsection{Artifact check-list (meta-information)}

{\small
\begin{itemize}

\item {\bf Algorithm: } Reinforcement learning algorithm for selecting the
  coherence mode of each accelerator at run-time based on the continuous
  monitoring of the system.

\item {\bf Program: } Multiple multi-threaded applications containing many
  accelerator invocations. These applications present a wide range of
  accelerator parallelism and workload sizes.

\item {\bf Compilation: } Automated cross-compilation for the SPARC processors
  in the SoC prototypes on FPGA. The compilation includes Linux and the test
  programs.
  
\item {\bf Run-time environment: } SoC prototypes on FPGA: Linux 5.1 SMP. Host
  machine for using ESP: either Docker or one of the OS supported by ESP,
  i.e. CentOS 7, Ubuntu 18.04 or Red Hat Enterprise Linux 7.8.

\item {\bf Hardware: } proFPGA UltraScale XCVU440 Prototyping Board.

\item {\bf Metrics: } Execution time and off-chip memory accesses.

\item {\bf Output: } CSV files with detailed results for each accelerator
  invocation.

\item {\bf Experiments: } Accelerators running in isolation with different
  coherence modes (Fig. 2), accelerators running in parallel with different
  coherence modes (Fig. 3), comparison of \cohmeleon to other solutions
  (design-time, run-time) on 7 different SoCs (Fig. 5,6,9), results with varying
  training iterations (Fig. 8).

\item {\bf How much disk space required (approximately)?: } Up to 64 GB if
  reproducing all experiments in the paper.

\item {\bf How much time is needed to prepare workflow (approximately)? }
  Setting up ESP takes 2-3 hours assuming all required tools are already
  installed. The generation of each FPGA bitstream takes up to 5 hours due to
  the large size of the target FPGA.

\item {\bf How much time is needed to complete experiments (approximately)? }
  Around 2 hours per experiment.

\item {\bf Publicly available? } Yes: complete source code and expected
  results.

\item {\bf Code licenses (if publicly available)?} Apache 2.0.

\item {\bf Archived (provide DOI)?: } Yes: 10.5281/zenodo.5150725.

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}
\label{sec:access}

We integrated \cohmeleon in ESP and we released it on GitHub
(\url{https://github.com/jzuckerman/esp/tree/cohmeleon}) and on Zenodo
(\url{https://doi.org/10.5281/zenodo.5150725}).
%
The most relevant directories and files for the integration and evaluation of \cohmeleon
are the following:

\begin{itemize}

\item \texttt{accelerators/}: Accelerators used in the experiments.

\item \texttt{soft/common/apps/examples/}: Applications for the case study SoCs
  and the motivation section results.

\item \texttt{socs/}: SoC design folders. The SoCs used for the experiments are
  labeled with the prefix \texttt{profpga-xcvu440-}. All \textit{Make} commands
  should be issued from these design folders. Each folder comes with scripts and
  configuration files for running the experiments.

\item \texttt{results/}: Expected results in CSV format.

\item \texttt{soft/common/drivers/linux/libesp/rl.h}: Core implementation of the
  \cohmeleon reinforcement-learning algorithm.
  
\item \texttt{rtl/sockets/csr/esp\_tile\_csr.vhd}: Core implementation of the
  ESP hardware monitoring system used by \cohmeleon.

\item \texttt{soft/common/drivers/linux/esp/esp.c}: Changes to the ESP device
  driver for accelerators to enable \cohmeleon.

\item \texttt{soft/common/drivers/linux/libesp/libesp.c}: Changes to
  the ESP API for accelerator invocation to enable \cohmeleon.

\end{itemize}

\subsubsection{Hardware dependencies}

proFPGA UltraScale XCVU440 Prototyping Board
(\url{https://www.profpga.com/products/fpga-modules-overview/virtex-ultrascale-based/profpga-xcvu440})
with four DDR4 daughter cards, a gigabit Ethernet interface daughter card, and a
multi-interface daughter card.
\cohmeleon will also work with any of the other FPGA boards
supported by ESP. We used the XCVU440 board because it has the largest FPGA
and is the only one with support for up to 4 memory channels.

\subsubsection{Software dependencies}

The software dependencies of ESP are described in the ``How to setup'' guide
(\url{https://esp.cs.columbia.edu/docs/setup/setup-guide/}), specifically in the
sections ``Software packets'', ``CAD tools'', ``Environment variables'', and
``Docker'' for users interested in using the ESP Docker image. In terms of CAD tools,
evaluating \cohmeleon requires only Xilinx Vivado 2019.2 and Cadence Stratus HLS
20.24 (other versions of Stratus should work too).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Installation}

The installation of ESP is described in the ``How to setup'' guide
(\url{https://esp.cs.columbia.edu/docs/setup/setup-guide/}), specifically in the
sections ``ESP repository'', ``Software toolchain'', and ``Docker''.  Evaluating
\cohmeleon requires cloning the fork of ESP listed in Section~\ref{sec:access}
and checking out the \texttt{cohmeleon} branch. Additionally, only the toolchain
for the LEON3 processor needs to be installed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

We encourage anyone attempting to use \cohmeleon to first familiarize themselves
with ESP. The resources available on the ESP website
(\url{https://esp.cs.columbia.edu/resources/}) include several hands-on tutorial
guides, the recordings of conference tutorials, and an overview paper.

\begin{enumerate}

\item \textbf{Run HLS}. Generate the RTL implementation of the accelerators. From any
  of the \texttt{socs/proFPGA-xcvu440-*/} folders, run \\ \texttt{make
    <acc\_name>-hls} for all the following accelerators:
  \\ \texttt{cholesky\_stratus}, \texttt{conv2d\_stratus}, \texttt{fft\_stratus},
  \texttt{gemm\_stratus},\\ \texttt{mriq\_stratus}, \texttt{nightvision\_stratus},
  \texttt{sort\_stratus}, \\ \texttt{svhn\_autoenc\_hls4ml},
  \texttt{svhn\_mlp\_hls4ml}, \texttt{synth\_stratus},
  \\ \texttt{vitdodec\_stratus}.


\item \textbf{Generate FPGA Bitstream}. In each \texttt{socs/proFPGA-xcvu440-*/}
  SoC design folder, run the following:

  \begin{itemize}

  \item \texttt{make esp-config}: Apply a predefined SoC configuration, which
    can be visualized by running \texttt{make esp-xconfig}.

  \item \texttt{make vivado-syn}: Generate the FPGA bitstream. This step can
    take several hours.

  \end{itemize}
  
  There is a design folder for each of the 7 SoCs used for the experiments:
  \begin{itemize}
  \item \texttt{profpga-xcvu440-12synth} : SoC0
  \item \texttt{profpga-xcvu440-7synth} : SoC1
  \item \texttt{profpga-xcvu440-9synth} : SoC2
  \item \texttt{profpga-xcvu440-16synth} : SoC3
  \item \texttt{profpga-xcvu440-10acc} : SoC4, also used for accelerator
    execution in isolation experiment (Fig. 2)
  \item \texttt{profpga-xcvu440-autonomous-driving} : SoC5 
  \item \texttt{profpga-xcvu440-computer-vision} : SoC6
  \item \texttt{profpga-xcvu440-12acc} : Used for accelerator execution in
    parallel experiment (Fig. 3), subsequently referred to as SoC7
\end{itemize} 

\item \textbf{Build Software}.

  \begin{itemize}

    \item \texttt{make linux}: Compile Linux for the Leon3 processor, and create
      Linux image for the experiments on FPGA.

    \item \texttt{make apps-cohmeleon}: Compile the applications required for
      the \cohmeleon experiments, and copy all executables, scripts, and data to
      the root-file system that gets included in the Linux image
      (\texttt{soft-build/leon3/sysroot}).

    \item \texttt{make linux}: Always re-run this target after modifying the
      content of the root file system.

  \end{itemize}   

\item \textbf{Deploy on FPGA}.

  \begin{itemize}

  \item \texttt{make fpga-program}: Program the FPGA with the SoC bitstream.

  \item \texttt{make fpga-run-linux}: Boot Linux on the SoC deployed on
    FPGA. Once the boot reaches the login prompt, log in with the username
    \texttt{root} and the password \texttt{openesp}.

  \end{itemize}

Deploying the bitstream and compiled software on the FPGA, as well as running
the experiments described in the next steps, requires proper connections  to the
FPGA. The main communication link is Ethernet, which is used for transferring
the Linux image onto the FPGA. After booting Linux on the FPGA, the same
Ethernet link enables the use of \texttt{ssh} and \texttt{scp}. In addition, it
is possible to establish a connection the UART port in order to monitor the
terminal outputs of the programs executing on the FPGA. Detailed instructions on
the FPGA setup can be found in the ESP ``How to: design a single-core SoC"
tutorial (\url{https://esp.cs.columbia.edu/docs/singlecore/singlecore-guide/}),
specifically in the sections ``Debug link configuration", ``UART interface", and
``SSH".
  
\item \textbf{Run Experiments}. After the login, navigate to the following
  directories to launch the experiment scripts for each SoC. Scripts and outputs
  are described in Section \ref{sec:eval}.
 
 \begin{itemize}
 \item \texttt{profpga-xcvu440-<N>synth} :\\ 
\texttt{/applications/test/}
 \item \texttt{profpga-xcvu440-10acc} : \\
 \texttt{/examples/multiacc/}\\ 
\texttt{/examples/single\_acc\_coh}  
 \item \texttt{profpga-xcvu440-autonomous-driving} :\\
 \texttt{/examples/auton\_driving/}
 \item \texttt{profpga-xcvu440-computer-vision} :\\
 \texttt{/examples/comp\_vision/}
 \item \texttt{profpga-xcvu440-12acc} :  \\
\texttt{/examples/parallel\_acc\_coh} 
 \end{itemize}  

 Output files of each experiment can be copied
  from the FPGA using \texttt{scp}.

\item \textbf{Process Data}. We provide scripts to process the experiments'
  outputs and produce the results presented in the paper, as described in
  Section \ref{sec:eval}.

\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagebreak
\subsection{Evaluation and expected results}
\label{sec:eval}

We provide the following scripts to execute the experiments presented in the
paper:

\begin{itemize}

\item \texttt{single\_acc\_coh.sh}: Reproduce the results in Fig. 2. Output
  file: \texttt{single\_acc\_coh.csv}. \texttt{(SoC4)}

\item \texttt{parallel\_acc\_coh.sh}: Reproduce the results in Fig. 3. Output
  file: \texttt{parallel\_acc\_coh\_devices.csv}. \texttt{(SoC7)}

\item \texttt{cohmeleon\_eval.sh}: Reproduce the results in Fig. 5, 7, 9. Output
  file: \texttt{<app\_name>\_phases.csv}, which reports the execution time and
  memory accesses for each phase of the application. These files can be passed
  to the script \texttt{process\_results.py} to produce the results of Fig. 9.
  Selected phases can be used to produce the results from Fig. 5. The coherence
  mode selected for each accelerator invocation is reported, along with
  statistics, in \texttt{<app\_name>\_devices.csv}. This can be used to
  reproduce the results in Fig. 7. \texttt{(SoCs 0, 1, 2, 3, 4, 5, 6)}

\item \texttt{training\_time.sh} : This script trains \cohmeleon over the course
of 10, 30, and 50 iterations, and records the performance after each iteration.
The script outputs 3 files, \texttt{training\_10.csv}, \texttt{training\_30.csv},
and \texttt{training\_50.csv}. These results can be passed to the script
\texttt{process\_training.py} to extract the results for Fig. 8. \texttt{(SoC0)}
\end{itemize}

The results for each figure in the paper are included in the \texttt{results}
folder of the repository. There is one CSV file for each figure.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiment customization}

The reward function can be tuned by changing the coefficients in the last line
before the return of \texttt{calculate\_reward()} in the \texttt{rl.h} header
file. After recompiling the applications and redeploying Linux on the FPGA, the
new model parameters can be tested with the \texttt{cohmeleon\_eval.sh}
script. Repeating these steps for multiple sets of coefficients will produce the
results in Fig. 6.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

